Improving Neural Language Modeling via Adversarial Training

Recently, substantial progress has been made in language modeling by using deep neural networks. However, in practice, large scale neural language models have been shown to be prone to overfitting. In this paper, we present a simple yet highly effective adversarial training mechanism for regularizing neural language models. The idea is to introduce adversarial noise to the output embedding layer while training the models. We show that the optimal adversarial noise yields a simple closed-form solution, thus allowing us to develop a simple and time efficient algorithm. Theoretically, we show that our adversarial mechanism effectively encourages the diversity of the embedding vectors, helping to increase the robustness of models. Empirically, we show that our method improves on the single model state-of-the-art results for language modeling on Penn Treebank (PTB) and Wikitext-2, achieving test perplexity scores of 46.01 and 38.07, respectively. When applied to machine translation, our method improves over various transformer-based translation baselines in BLEU scores on the WMT14 English-German and IWSLT14 German-English tasks.

==> tex/bakup.tex <==

\paragraph{Including Uncertainty in Softmax}

For the Softmax layer, we have a context matrix $C$ and a word embedding matrix $W$. Now, we have converted each word embedding into a Gaussian distribution, so we rewrite the embedding matrix as $(W_\mu, W_\sigma)$. Once we want to use both mean and variance during evaluation, we should change the structure of Softmax layer. We make a new Softmax layer as  $p(\cdot | c) = \sum_{i=1}^{n}{\pi_i \frac{\exp^{c \cdot (W_{\mu, \cdot}+ b_i W_{\sigma, \cdot})}}{Z}}$ where $p_i = \mathcal{N}(b_i; \bm 0, \bm 1)$. $\{b_i\}_{i=1}^{n}$ are $n$ particles drawn from normal distribution. Currently, we draw $n$ particles using SVGD before training in the beginning, and fix its value during training. We also fix the value of the variance, since we find it is hard to train variance. \textbf{In our experiments, we now fix all the variance to be $0.3$. $n$ is set to 5.}

Before this, I have already try several other approaches: 1. Only including noise during training for softmax layer, and using the mean value during evaluation. (doesn't work) 2. Including noise during training for softmax layer for training and evaluation. (doesn't work) 3. Drawing random $\{b_i\}_{i=1}^{n}$ during training, and using normal Softmax during evaluation. (doesn't work) 4. Only using the above method during training, and using the normal Softmax during evaluation. (doesn't work) 5. Mixing $n$ particles before Softmax. (doesn't work, since it is the same as only using mean) 


\section{Gaussian Embeddings}
\red{what would be the best way to model a neural network with distributions as input?}

For each word $w$ in the dataset, the distribution of
its latent meaning $\theta \sim p_w(\theta)$ (embedding), we parameterize $p_w$ as a Gaussian distribution, 
$$
p_w(\theta) = \normal(\theta; \mu_w, \sigma_w^2),
$$
with mean $\mu_w$ and variance $\sigma_w^2$.

Given a sequence of words $\{w_{-i}, w_i\}$, 
we would like to maximize the log-likelihood, 
$$
\log p(w_i |w_{-i}) = \log \int p(w_i|c) p_\phi(c|w_{-i}) dc,
$$
where $c$ 

With the reparameterization trick, 
the Gaussian embeddings 
$\hat w = \mu + \sigma\odot \epsilon, ~~\epsilon \sim \normal(0, 1)$. Let $c$ be the
output of the RNN, and $\hat{w}_i$ be the noisy embeddings of the $i$-th work,
the soft probability can be written as 
$$
\log p(w_i| c) = \log \frac{\exp(c^\top \hat{w}_i)}{\sum_j \exp(c^\top \hat{w}_j)} = c^\top \hat{w}_i - \log \sum_j \exp(c^\top \hat{w}_j).
$$
By calculating the gradient w.r.t. $\mu_i,\sigma_i\in \R^d$, we have
$$
\begin{aligned}
\frac{\partial \log p(w_i |c)}{\partial \mu_i} &= c \bigg( 1 - \frac{1}{\sum_j \exp(c^\top \hat{w}_j)} \bigg) \approx c , \\
\frac{\partial \log p(w_i |c)}{\partial \sigma_i} &= (c\odot\epsilon) \bigg( 1 - \frac{1}{\sum_j \exp(c^\top \hat{w}_j)} \bigg) \approx c \odot \epsilon.
\end{aligned}
$$
The gradient of the variance term could be very noisy if the magnitude of the context representation 
is large. 

\red{easy fix}: parameterize the variance with another neural network. Specifically, 
we train a neural network $V(\mu_i, f_i)$, which takes the embedding $\mu_i$ and word frequency $f_i$ as input and output the variance estimation.

\paragraph{Breaking the softmax bottleneck with random samples?}
The objective is to maximize the log-likelihood given the contex
$$
\log p(w_i | w_{-i}) = \log \int p(w_i |c) p_\theta(c|w_{-i}) dc,
$$
where $c$ represents context, $p_\theta(c|w_{-i})$ is a recurrent neural network, and 
$$
p(w_i|c) = \frac{\D(p(w_i), p(c|w_{-i}))}{\sum_j \D(p(w_j), p(c|w_{-i}))},
% \frac{\exp(w_i^\top c)}{\sum_j \exp(w_j^\top c)},
$$

The empirical estimation of the log-likelihood can be written as
$$
\log p(w_i | w_{-i}) = \log \E_{c \sim p(c|w_{-i})} = \log \E_{c\sim  p(c|w_{-i})}  \frac{\exp(w_i^\top c)}{\sum_j \exp(w_j^\top c)}.
$$

For simplicity, we explore the following two divergence between distributions, 
\paragraph{Expected Likelihood} The energy between Gaussian is defined as
$$
\D_{energy}(p_i, p_j) = \int \normal(\mu_i, \Sigma_i)\normal(\mu_j, \Sigma_j) dx.
$$
The logarithm of the energy is
$$
\log e(p_i, p_j) = -\frac{1}{2}\log \det(\Sigma_i +\Sigma_j) 
-\frac{1}{2}(\mu_i -\mu_j)^\top(\Sigma_i+\Sigma_j)^{-1}(\mu_i -\mu_j) - \frac{d}{2}\log 2\pi.
$$
\textbf{Remark} Controlling the bottom eigenvalues of the covariance is
especially important, the $\log\det$ term can give very high scores to small
covariances that dominating the rest of the energy.


\paragraph{Wasserstein Distance}
$$
\D_{W_2}(p_i, p_j) = (\mu_i -\mu_j)^\top(\mu_i -\mu_j) +
\trace(\Sigma_i + \Sigma_j - 2(\Sigma_j^{1/2}\Sigma_i \Sigma_j^{1/2})^{1/2})
$$

\section{Related Work}
\begin{enumerate}  
    \item MOS \citep{yang2017breaking}, DOC (very similar to MOS) \citep{takase2018doc}
    \item Sigsoftmax: Reanalysis of the Softmax Bottleneck \citep{kanai2018sigsoftmax} 
    \item Noisin \citep{dieng2018noisin}
    \item Gaussian word embedding \citep{vilnis2014word}
\end{enumerate}
